Shintani theta lifts of harmonic Maass forms

We define a regularized Shintani theta lift which maps weight $2k+2$ ($k \in \Z, k \geq 0$) harmonic Maass forms for congruence subgroups to (sesqui-)harmonic Maass forms of weight $3/2+k$ for the Weil representation of an even lattice of signature $(1,2)$. We show that its Fourier coefficients are given by traces of CM values and regularized cycle integrals of the input harmonic Maass form. Further, the Shintani theta lift is related via the $\xi$-operator to the Millson theta lift studied in our earlier work. We use this connection to construct $\xi$-preimages of Zagier's weight $1/2$ generating series of singular moduli and of some of Ramanujan's mock theta functions.

==> delta_pre.tex <==
\section{A $\Delta_{2k+2}$-preimage for the Shintani schwarz function}

For $X \in V$ and $\tau,z \in \H$ with $Q_{X}(z) \neq 0$ we let
\[
\eta(X,\tau,z) = -\frac{ 2^{k-1}N^{k+1}}{Q_{X}^{k+1}(z)}\int_{|p_{z}(X)|}^{\infty}\left(\frac{1}{2}t^{2}-(X,X)\right)^{k}\erfc\left(\sqrt{\pi v}t\right)dt.
\]
It is smooth on its domain. For the computation of the Fourier coefficients of the Shintani lift we will need the following differential equations and growth estimates for $\eta(X,\tau,z)$.


\begin{lem}
	\begin{enumerate}
		\item For $Q_{X}(z) \neq 0$ we have
	\begin{align*}
	\xi_{2k+2} \eta(X,\tau,z) = \frac{\sqrt{N}}{2}Q_{X}^{k}(z) \sgn(p_{z}(X))\erfc\left(\sqrt{\pi v}|p_{z}(X)|\right)
	\end{align*}
	and
	\[
	\Delta_{2k+2} \eta(X,\tau,z) = \varphi_{Sh}^{0}(X,\tau,z).
	\]
		\item For $Q(X) > 0$ the functions $\eta(X,\tau,z)$ and $\xi_{2k+2}\eta(X,\tau,z)$ are square exponentially decreasing as $y \to 0$ and $y \to \infty$, uniformly in $x$, and as $x \to \infty$, uniformly in $y$.
		\item For $Q(X) < 0$ such that the stabilizer $\overline{\Gamma}_{X}$ is infinite cyclic, the functions $\eta(X,\tau,z)$ and $\xi_{2k+2}\eta(X,\tau,z)$ are square exponentially decreasing at the boundary of $\Gamma_{X} \setminus \H$.
	\end{enumerate}
\end{lem} 

\begin{proof}
	\begin{enumerate}
	\item This follows by a straightforward calculation using the rules \eqref{eq:diffpQR}.

	\item For $X = \left(\begin{smallmatrix}x_{2} & x_{1} \\ x_{3} & -x_{2}\end{smallmatrix} \right)$ with $Q(X) > 0$ we have $x_{3} \neq 0$ and 
	\[
	-\pi p_{z}^{2}(X) = -\pi \left( \frac{N(x_{3}x-x_{2})^{2}+q(X)}{\sqrt{N}x_{3}y} + \sqrt{N}x_{3}y\right)^{2}.
	\]
	This immediatly implies the claimed decay of $\eta(X,\tau,z)$ and $\xi_{2k+2}\eta(X,\tau,z)$.
	\item Let $Q(X) = m < 0$ such that $\overline{\Gamma}_{X}$ is infinite cyclic. By conjugation with a matrix in $\SL_{2}(\R)$ we can assume that $X$ has the form $X = \sqrt{\frac{|m|}{N}}\left(\begin{smallmatrix}1 & 0 \\ 0 & - 1 \end{smallmatrix}\right)$.
	Then the stabilizer of $X$ is given by
	\[
	\overline{\Gamma}_{X} = \left\{\begin{pmatrix}\varepsilon  & 0 \\ 0 &\varepsilon^{-1}\end{pmatrix}^{n}: n \in \Z\right\}
	\]
	for some $\varepsilon > 1$, and a fundamental domain for $\Gamma_{X}\setminus \H$ is given by the set $\{z \in \H: 1 \leq |z| \leq \varepsilon^{2}\}$. The two semi-arcs $|z| = 1$ and $|z| = \varepsilon^{2}$ are identified via $\Gamma_{X}$, so letting $z$ go to the boundary of $\Gamma_{X}\setminus \H$ means letting $y$ go to $0$ with $x$ being bounded away from $0$. Explicitly, we have $p_{z}(X) = 2\sqrt{|m|}\,\frac{x}{y}$. The claimed decay of $\eta(X,\tau,z)$ and $\xi_{2k+2}\eta(X,\tau,z)$ at the boundary of $\Gamma_{X}\setminus \H$ is now easy to check.
	\end{enumerate}
\end{proof}


